Asymptotic Validity and Finite-Sample Properties of Approximate Randomization Tests

Randomization tests rely on simple data transformations and possess an appealing robustness property. In addition to being finite-sample valid if the data distribution is invariant under the transformation, these tests can be asymptotically valid under a suitable studentization of the test statistic, even if the invariance does not hold. However, practical implementation often encounters noisy data, resulting in approximate randomization tests that may not be as robust. In this paper, our key theoretical contribution is a non-asymptotic bound on the discrepancy between the size of an approximate randomization test and the size of the original randomization test using noiseless data. This allows us to derive novel conditions for the validity of approximate randomization tests under data invariances, while being able to leverage existing results based on studentization if the invariance does not hold. We illustrate our theory through several examples, including tests of significance in linear regression. Our theory can explain certain aspects of how randomization tests perform in small samples, addressing limitations of prior theoretical results.

==> preamble.tex <==

\usepackage{amsmath, mathtools, bbm}
%\usepackage{graphics}
\RequirePackage{graphicx}
\usepackage{tikz}
\usetikzlibrary{patterns,arrows,decorations.pathreplacing}

\usepackage{newtxtext}
\usepackage[subscriptcorrection]{newtxmath}
\usepackage{color}
%\usepackage{natbib}

% \graphicspath{{./art/}}

\usepackage[plain,noend]{algorithm2e}

\makeatletter
\renewcommand{\algocf@captiontext}[2]{#1\algocf@typo. \AlCapFnt{}#2} % text of caption
\renewcommand{\AlTitleFnt}[1]{#1\unskip}% default definition
\def\@algocf@capt@plain{top}
\renewcommand{\algocf@makecaption}[2]{%
  \addtolength{\hsize}{\algomargin}%
  \sbox\@tempboxa{\algocf@captiontext{#1}{#2}}%
  \ifdim\wd\@tempboxa >\hsize%     % if caption is longer than a line
    \hskip .5\algomargin%
    \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}% then caption is not centered
  \else%
    \global\@minipagefalse%
    \hbox to\hsize{\box\@tempboxa}% else caption is centered
  \fi%
  \addtolength{\hsize}{-\algomargin}%
}
\makeatother

%%% User-defined macros should be placed here, but keep them to a minimum.
\def\Bka{{\it Biometrika}}
\def\AIC{\textsc{aic}}
\def\T{{ \mathrm{\scriptscriptstyle T} }}
\def\v{{\varepsilon}}

%\addtolength\topmargin{35pt}
\DeclareMathOperator{\Thetabb}{\mathcal{C}}

%% Errors 
\newcommand{\eps}{\varepsilon}
\newcommand{\heps}{\widehat\eps}
\newcommand{\hepsr}{\widehat{\eps^{\mathrm{o}}}}

%% Stats
\newcommand{\mE}{\mathbb{E}}
\newcommand{\mVar}{\mathbb{V}\mathrm{ar}}
\newcommand{\var}{\mathrm{var}}
\newcommand{\mCov}{\mathrm{cov}}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}

\newcommand{\myitemsep}{  \setlength\itemsep{-.15em} }
\newcommand\myeq[1]{\stackrel{\mathclap{\normalfont\mbox{\tiny{$\mathrm{#1}$}}}}{=}}
\newcommand\myapprox[1]{\stackrel{\mathclap{\normalfont\mbox{\tiny{$\mathrm{#1}$}}}}{\approx}}

\newcommand\myge[1]{\stackrel{\mathclap{\normalfont\mbox{\tiny{$\mathrm{#1}$}}}}{\ge}}
\newcommand\myle[1]{\stackrel{\mathclap{\normalfont\mbox{\tiny{$\mathrm{#1}$}}}}{\le}}
\newcommand\mysim[1]{\stackrel{\mathclap{\normalfont\mbox{\tiny{$\mathrm{#1}$}}}}{\sim}}
\newcommand\limeq[1]{\stackrel{\mathclap{\normalfont\mbox{\tiny{$#1$}}}}{\to}}
\newcommand{\ones}{\mathbf{1}}

%%%% THEOREMS
%% THEOREMS in the paper.
% \renewcommand{\gg}{\mathtt{g}\hspace{.7px}}
\renewcommand{\gg}{\mathrm{g}}
\newcommand{\GG}{G}
\newcommand{\GGnr}{\GG_{r, n}}
\newcommand{\hGGnr}{\hat\GG_{r, n}}

\newcommand{\Gall}{\mathcal{G}_n}
\newcommand{\Unif}{\mathrm{Unif}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\XXn}{\mathbb{X}^{(n)}}
\newcommand{\Am}{\langle A_m(\Gall) \rangle}

\newcommand{\phione}{\phi_{n}}
\newcommand{\phitwo}{\phi_{n}^{\mathrm{\text{two}}}}

\newcommand{\todo}[1]{\text{\textcolor{red}{xx TODO: #1 xx}}}
\newcommand{\note}[1]{\textcolor{blue}{xx NOTE: #1 xx}}
\newcommand{\commentEq}[1]{\quad\quad\footnotesize{\text{[{\em #1}]}}}
\newcommand{\Ind}{\mathbbm{1}}
\newcommand{\Indb}[1]{\mathbbm{1}\big\{#1\big\}}
\newcommand{\cc}{c}
\newcommand{\epsn}{\eps}
\newcommand{\epsr}{\eps^{\mathrm{o}}}

\newcommand{\yn}{Y^{n}}

\newcommand{\Yn}{\yn}
\newcommand{\Xn}{X^n}
\newcommand{\Xdomain}{\mathbb{X}^{n}}

\newcommand{\XnT}{X^{(n)\top}}
\renewcommand{\XnT}{X^\top}

\newcommand{\XXT}{(\XnT \Xn)^{-1} \XnT}

\newcommand{\hbeta}{\hat\beta_n}
\newcommand{\hbetar}{\hat{\beta}_n^{\mathrm{o}}}
\newcommand{\wpval}{\widehat{\mathrm{pval}}}
\newcommand{\tageq}[1]{\quad\quad\text{#1}}

\newcommand{\Tne}{\mathbf{S}_{n, \eps}}
\newcommand{\Tner}{\mathbf{S}_{n, \heps}}


\newcommand{\M}{\boldsymbol{\mathrm{M}}}
\newcommand{\Ve}{\mathbf{V}_\eps}
\newcommand{\VV}{\tilde V}
\newcommand{\Vx}{\mathbf{V}_{\mathrm{x}}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\B}{\mathbf{B}}

\newcommand{\FLn}{F_{\LamStud}}
\newcommand{\GR}{\mathbf{G}_{n,m}}

\newcommand{\lmax}{\lambda_{\max}}
\newcommand{\lmin}{\lambda_{\min}}
\newcommand{\trace}{\mathrm{tr}}

\newcommand{\dyad}{\mathsf{dyad}}

%% Leverage
\newcommand{\lev}{\bar\lambda_n}
\newcommand{\levv}{\bar\lambda_{n,2}}
\newcommand{\levI}{\bar\lambda_1(\CC^n)}
\newcommand{\levII}{\bar\lambda_2(\CC^n)}

%% CLUSTERS
%% Clusters
\newcommand{\ccc}{[\cc]}
\newcommand{\CC}{\mathrm{C}}

\newcommand{\jj}{\ccc}
\newcommand{\DD}{\mathbf{I}}
\newcommand{\DDR}{\mathbf{R}}
\renewcommand{\R}{\DDR}
\newcommand{\DDC}{\mathbf{C}}
\newcommand{\C}{\DDC}

\newcommand{\LamStud}{\Lambda_n^{s}}
\newcommand{\Tstud}{T_n^\mathrm{s}}
\newcommand{\LamMin}{\Lambda_{(1)}}
\newcommand{\DeltaMax}{\Delta_{(n)}}

\newcommand{\ConditionEClustPerm}{
  \frac{\max_{\cc\in[J_n]} \mE[s_\cc^2(\eps)] }{\min_{\cc'\in[J_n]} \mE[s_{\cc'}^2(\eps)]  } 
  }
  \newcommand{\ConditionES}{
      % \frac{\max_{i\in[n]}  \mE(\eps_i^2)}{\min_{j\in[n]} \mE(\eps_j^2)}
   \min\left\{ \sigma_n^*, \psi_n^* \right\}    
  }
  \newcommand{\ConditionESCluster}{
  p^3 \kappa_n^2 \kappa(\Qx \Ve \Qx^\top)~ \levII \sum_{\cc=1}^{J_n} n_\cc^2/n^2
  }
  
  \newcommand{\ConditionTwoWayCluster}{
  p^4 \kappa_n^2~\kappa(\Qx \Ve \Qx^\top)~\big(1/|\RR^n| +1/ |\CC^n|\big)
  }
    \newcommand{\ConditionPanel}{
  p^4 \kappa_n^2~\kappa(\Qx \Ve \Qx^\top)~\levv/ N
  }
%% NOTATION FOR X

\newcommand{\xj}{x_{\cdot j}}
\newcommand{\xpj}{x_{\cdot \pi(j)}}
\newcommand{\xk}{x_{\cdot k}}
\newcommand{\xrow}[1]{x_{#1\cdot}}

\newcommand{\barzc}{\overline{z_{\cc}}}
\newcommand{\barxc}{\overline{x_{\cc}}}
\newcommand{\barzcc}{\overline{z_{\cc}^2}}
\newcommand{\barxcc}{\overline{x_{\cc}^2}}
\newcommand{\normzc}{||z_{\cc}||^2}
\newcommand{\normxc}{||x_{\cc}||^2}
\newcommand{\xrowc}[1]{||X_{#1\cdot}||_F^2}
\newcommand{\xrowcc}[1]{||X_{#1\cdot}||_F^4}

% \newtheorem{procedure}{Procedure}
\newcommand{\ven}{v_{\eps,n}}


\newcommand{\vc}{c}
\newcommand{\gon}{\gamma_{0n}}
\newcommand{\nn}{\nonumber}

\newcommand{\Qx}{Q_{\mathrm{x}}}
 \newcommand{\Pn}{\mathbf{P}_{\mathrm{x}} }

 \newcommand{\Px}{\mathbf{H}_{\mathrm{x}} }
\newcommand{\Pxo}{\Px^{\mathrm{o} } }
\newcommand{\pp}{p}
\newcommand{\Sym}{\Pi}
%% Signs
\renewcommand{\ss}{s}


\newcommand{\DDU}{\mathbf{U}}
\newcommand{\Don}{\Delta_n^{\mathrm{o}}}
\newcommand{\zon}{\zeta_n^{\mathrm{o}}}


\newcommand{\TTne}{S_n}
\newcommand{\Tneh}{\todo{defunct: fix}}

%%   Positive-definite matrices
\newcommand{\Hx}{\Px}
\newcommand{\Id}{\mathbf{I}}
 \renewcommand{\S}{\mathbf{S}}
 \newcommand{\V}{\mathbf{V}}
\newcommand{\U}{\mathbf{U}}
\newcommand{\D}{\boldsymbol{\Delta}}

\newcommand{\Xin}{\Xi_{(n)}}

%% THEOREMS


\newcommand{\TheoremZero}{
Suppose that Assumptions~\eqref{A:Gall}-\eqref{A:degen}  hold for 
$\eps = (\eps_1, \ldots, \eps_n)$ and a test statistic $T_n$, for which $T_n=t_n(\eps)$ under some null hypothesis. 
%
Then, under Condition~\eqref{eq:C1}, 
$$
| \mE(\phione) - \mE(\phi_n^*) | \le 1/m + o(1)~.
$$
}


\newcommand{\TheoremOne}{
Suppose that Assumptions~\eqref{A:Gall}-\eqref{A:gon} and~\eqref{A:gammas}  hold for 
$\eps = (\eps_1, \ldots, \eps_n)$ and a test statistic $T_n$, for which $T_n=t_n(\eps)$ under some null hypothesis. Then, for any $n>0$,
\begin{equation}
|\mE(\phione) - \mE(\phi^*_n)| \le O(1/m) + O(m\gon) + O(m^2/ |\Gall|)  +  A(\gamma, m)\cdot O\big(\zeta_n^{2\gamma/(2+\gamma)}\big)~,
\end{equation}
whenever the null hypothesis is true. Here, $A(\gamma, m) = 8(1+\gamma) m^{(4+\gamma) / (2+\gamma)} = O(m^2)$. 
% The same result holds for the test using $\hbetar$, the restricted OLS estimator,  under Conditions~\eqref{C:var0}-\eqref{C:gammas}.
}


\newcommand{\TheoremPower}{
Suppose that Assumptions~\eqref{A:Gall}-\eqref{A:degen}  hold for 
$\eps$ and a test statistic $T_n$, for which $T_n=t_n(\eps)$ under some null hypothesis. 
Let $\sigma_n^2 = 2\mE[\mVar(t_n(G \eps)|\eps) ],~G\sim\Unif(\Gall)$, and consider a sequence of alternatives, $H_1: T_n = t_n(\eps) + \tau_n$. Then, 
for any sequence $\tau_n /\sigma_n\to\infty$,
$$
\mE(\phi_n) \to 1,~\text{if either invariance~\eqref{eq:invariant_hypothesis} holds or}~
P(|t_n(G\eps) - t_n(\eps)| > \tau_n/\sigma_n)\to0.
$$
Suppose, in addition, that Assumption~\eqref{A:gammas} holds, and there exists a non-decreasing function $q: \Real^+\to\Real^+$ such that 
$F_{\bar \Lambda_n}(l) - F_{\bar \Lambda_n}(-l)  \ge 1 - e^{-q(l) }$, for any $l > 0$.
Then, under the same conditions, it holds that
\begin{equation}
\mE(\phione) \ge  1 - O(m^2) e^{-q(\tau_n / 2\sqrt{2} \sigma_n)} - A(\gamma, m) \cdot O(\zeta_n^{2\gamma/(2+\gamma)}).\nonumber
\end{equation}
The expression for the two-sided test uses $|\tau_n| / \sigma_n$, but is otherwise identical.
% where $A(\gamma, m)$ and $\zeta_n^2$ are defined in~Theorem~\ref{thm:main}. 
% \end{longlist}
}

\newcommand{\TheoremPerm}{
For the linear model in~\eqref{eq:linear_model}, suppose that Assumptions~\eqref{A:X_eps2}, \eqref{A:gon}, \eqref{A:degen} hold true for the test
statistic functions $t_n$ and $t_n^s$. 
%
In the residual permutation test,  Condition~\eqref{eq:C1} for the unstudentized statistic $t_n$ reduces to
\begin{equation}\label{eq:C1_perm}
\frac{ \mE(|| \Pn \eps||^2/n)}{\mE(||\eps||^2/n)} \to 0.~\tag{C1'}
\end{equation}
Under~\eqref{eq:invariant_hypothesis_error}, the invariant hypothesis of 
exchangeability,  this condition is satisfied if $p/n = o(1)$.
%
Under~\eqref{eq:limit_hypothesis_error}, the limit hypothesis, Condition~(C1') is true without additional assumptions, and also implies that Condition (C1) is true for the studentized statistic $t_n^s$ as well.
% the same result holds true under the studentized statistic $ t_n^s(\cdot)$ of Equation~\eqref{eq:linear_Tn2}, provided that the  limit hypothesis~\eqref{eq:limit_hypothesis_error} is true as well.
}

\newcommand{\TheoremS}{
For the linear model in~\eqref{eq:linear_model}, suppose that Assumptions~\eqref{A:X_eps2}, \eqref{A:gon}, \eqref{A:degen} hold true for the test
statistic functions $t_n$ and $t_n^s$. 
In the residual sign test,  Condition~\eqref{eq:C1} for the unstudentized statistic $t_n(\cdot)$ reduces to
\begin{equation}\label{eq:C1_sign}
\ConditionES~\lev p/n  = o(1).\tag{C1''}
\end{equation}
Under~\eqref{eq:limit_hypothesis_error}, this is also sufficient to satisfy Condition~\eqref{eq:C1} for the studentized statistic $t_n^s$.
}

\newcommand{\TheoremPermS}{
%For the linear model in~\eqref{eq:linear_model} let $\eps\myeq{d} \gg\eps \mid X$ for all $\gg\in\Gall^{\pp+\ss}$ and $X\in\XXn$,~$n>0$, such that Assumptions~\eqref{A:X_eps2}-\eqref{A:gon} are satisfied.  
%%%%
For the linear model in~\eqref{eq:linear_model}, let invariance~\eqref{eq:fs_invariant_X} hold under $\Gall =\Gall^\pp$. 
Suppose that Assumptions~\eqref{A:X_eps2}, \eqref{A:gon}, \eqref{A:degen} are satisfied, 
and that $p/n=o(1)$. 
Then, Condition~\eqref{C:var} is satisfied and the residual randomization test, $\phi_n$,  sampling transformations from $\Gall^{\pp+\ss}$ is asymptotically valid for the linear hypothesis.
}


